Retrieval-augmented Prompt Learning for Pre-trained Foundation Models

The pre-trained foundation models (PFMs) have become essential for facilitating large-scale multimodal learning. Researchers have effectively employed the ``pre-train, prompt, and predict'' paradigm through prompt learning to induce improved few-shot performance. However, prompt learning approaches for PFMs still follow a parametric learning paradigm. As such, the stability of generalization in memorization and rote learning can be compromised. More specifically, conventional prompt learning might face difficulties in fully utilizing atypical instances and avoiding overfitting to shallow patterns with limited data during the process of fully-supervised training. To overcome these constraints, we present our approach, named RetroPrompt, which aims to achieve a balance between memorization and generalization by decoupling knowledge from mere memorization. Unlike traditional prompting methods, RetroPrompt leverages a publicly accessible knowledge base generated from the training data and incorporates a retrieval mechanism throughout the input, training, and inference stages. This enables the model to actively retrieve relevant contextual information from the corpus, thereby enhancing the available cues. We conduct comprehensive experiments on a variety of datasets across natural language processing and computer vision tasks to demonstrate the superior performance of our proposed approach, RetroPrompt, in both zero-shot and few-shot scenarios. Through detailed analysis of memorization patterns, we observe that RetroPrompt effectively reduces the reliance on rote memorization, leading to enhanced generalization.

==> case_table.tex <==
\begin{table*}
\centering
\caption{Case examples of Top-3 and Bottom-3 memorized instance of {ours} from trainset of SST-2.
}
\label{table.vis.sst}
\resizebox{0.95\textwidth}{!}{
% \begin{small}
\begin{tabular}{lp{0.5cm}p{1.3cm}<{\centering}lp{0.5cm}p{1.3cm}<{\centering}}
\toprule
\multicolumn{3}{c}{\textbf{Negative}} & \multicolumn{3}{c}{\textbf{Positive}} \\
\cmidrule(lr){1-3} \cmidrule(lr){4-6}
\textbf{Content} &\textbf{Mem} & {$F(p_{k\text{NN}})$} & \textbf{Content} &\textbf{Mem} & $F(p_{k\text{NN}})$\\
\midrule
\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}
\colorbox{white!0}{\parbox{0.45\textwidth}{
\colorbox{red!0}{\strut Although} \colorbox{red!0}{\strut god} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut great} \colorbox{red!0}{\strut addressed} \colorbox{red!0}{\strut interesting} \colorbox{red!0}{\strut matters} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut identity} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut heritage,} \colorbox{red!0}{\strut it's} \colorbox{red!0}{\strut hard} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut shake} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut feeling} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut intend} \colorbox{red!0}{\strut to} 
\colorbox{red!0}{\strut be} 
\colorbox{red!0}{\strut a} 
\colorbox{red!0}{\strut different} 
\colorbox{red!0}{\strut kind} 
\colorbox{red!0}{\strut of} 
\colorbox{red!0}{\strut film.} 
}}}
\end{CJK*} 
& 0.066 & 1.17 &
\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
\colorbox{red!0}{\strut A} \colorbox{red!0}{\strut b-movie} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut sit} \colorbox{red!0}{\strut through,} \colorbox{red!0}{\strut enjoy} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut certain} \colorbox{red!0}{\strut level} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut forget.}
}}}\end{CJK*} 
& 0.020 & 0.18\\ 
% \midrule
\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
\colorbox{red!0}{\strut A} \colorbox{red!0}{\strut standard} \colorbox{red!0}{\strut police-oriented} \colorbox{red!0}{\strut drama} \colorbox{red!0}{\strut that,} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut deniro's} \colorbox{red!0}{\strut participation,} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut likely} \colorbox{red!0}{\strut wound} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut tnt} \colorbox{red!0}{\strut original.} 
}}}
\end{CJK*} 
& 0.011 & 1.48 &
\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
\colorbox{red!0}{\strut A} \colorbox{red!0}{\strut film} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut appreciated} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut those} \colorbox{red!0}{\strut willing} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut endure} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut extremely} \colorbox{red!0}{\strut languorous} 
\colorbox{red!0}{\strut rhythms,} 
\colorbox{red!0}{\strut waiting} 
\colorbox{red!0}{\strut for} 
\colorbox{red!0}{\strut happiness} 
\colorbox{red!0}{\strut is} 
\colorbox{red!0}{\strut ultimately} 
\colorbox{red!0}{\strut thoughtful} 
\colorbox{red!0}{\strut without} 
\colorbox{red!0}{\strut having} 
\colorbox{red!0}{\strut much} 
\colorbox{red!0}{\strut dramatic} 
\colorbox{red!0}{\strut impact.} 
}}}\end{CJK*}
& 0.010 & 0.43 \\ 
% \midrule
\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
\colorbox{red!0}{\strut A} \colorbox{red!0}{\strut hit} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut miss} \colorbox{red!0}{\strut affair,} \colorbox{red!0}{\strut consistently} \colorbox{red!0}{\strut amusing} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut outrageous} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut funny} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut cho} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut intended} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut imaginative} \colorbox{red!0}{\strut as} 
\colorbox{red!0}{\strut one} 
\colorbox{red!0}{\strut might} 
\colorbox{red!0}{\strut have} 
\colorbox{red!0}{\strut hoped.} 
 
}}}
\end{CJK*} 
& 0.010 &  2.74 &
\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
\colorbox{red!0}{\strut What's} \colorbox{red!0}{\strut invigorating} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut it} 
\colorbox{red!0}{\strut doesn't} 
\colorbox{red!0}{\strut give} 
\colorbox{red!0}{\strut a} 
\colorbox{red!0}{\strut damn.} 
}}}\end{CJK*}
& 0.003 & 0.06 \\ 
\midrule
\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
\colorbox{red!0}{\strut It's} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut loathsome} \colorbox{red!0}{\strut movie,} \colorbox{red!0}{\strut it}  
\colorbox{red!0}{\strut really}  
\colorbox{red!0}{\strut is}  
\colorbox{red!0}{\strut and}  
\colorbox{red!0}{\strut it}  
\colorbox{red!0}{\strut makes}  
\colorbox{red!0}{\strut absolutely}  
\colorbox{red!0}{\strut no}  
\colorbox{red!0}{\strut sense.}  
}}}\end{CJK*} 
& 0.00 & 0.00 &
\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
\colorbox{red!0}{\strut A} \colorbox{red!0}{\strut fun} \colorbox{red!0}{\strut family} \colorbox{red!0}{\strut movie} \colorbox{red!0}{\strut that's} \colorbox{red!0}{\strut suitable} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut ages--} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut movie} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut make} \colorbox{red!0}{\strut you} 
\colorbox{red!0}{\strut laugh,} 
\colorbox{red!0}{\strut cry} 
\colorbox{red!0}{\strut and} 
\colorbox{red!0}{\strut realize,} 
\colorbox{red!0}{\strut `it's} 
\colorbox{red!0}{\strut never} 
\colorbox{red!0}{\strut too} 
\colorbox{red!0}{\strut late} 
\colorbox{red!0}{\strut to} 
\colorbox{red!0}{\strut believe} 
\colorbox{red!0}{\strut in} 
\colorbox{red!0}{\strut your} 
\colorbox{red!0}{\strut dreams.'} 
}}}\end{CJK*} 
& 0.00 & 0.00 \\ 
% \midrule
\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
\colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is}
\colorbox{red!0}{\strut that}
\colorbox{red!0}{\strut rare}
\colorbox{red!0}{\strut combination}
\colorbox{red!0}{\strut of}
\colorbox{red!0}{\strut bad}
\colorbox{red!0}{\strut writing,}
\colorbox{red!0}{\strut bad}
\colorbox{red!0}{\strut direction}
\colorbox{red!0}{\strut and}
\colorbox{red!0}{\strut bad}
\colorbox{red!0}{\strut acting}
\colorbox{red!0}{\strut --}
\colorbox{red!0}{\strut the}
\colorbox{red!0}{\strut trifecta}
\colorbox{red!0}{\strut of}
\colorbox{red!0}{\strut badness.}
}}}\end{CJK*} 
& 0.00 & 0.00 &
\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
\colorbox{red!0}{\strut It's} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut cool} \colorbox{red!0}{\strut event} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut whole} \colorbox{red!0}{\strut family.} 
}}}\end{CJK*}
& 0.00 & 0.00 \\ 
% \midrule
\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
\colorbox{red!0}{\strut This} \colorbox{red!0}{\strut thing} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut virtually} \colorbox{red!0}{\strut unwatchable.} 
}}}\end{CJK*}
& 0.00 & 0.00 &
\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
\colorbox{red!0}{\strut Good} \colorbox{red!0}{\strut fun,} \colorbox{red!0}{\strut good} \colorbox{red!0}{\strut action,} \colorbox{red!0}{\strut good} \colorbox{red!0}{\strut acting,} \colorbox{red!0}{\strut good} \colorbox{red!0}{\strut dialogue,} \colorbox{red!0}{\strut good} \colorbox{red!0}{\strut pace,} \colorbox{red!0}{\strut good} \colorbox{red!0}{\strut cinematography.} 
}}}\end{CJK*} 
& 0.00 & 0.00 \\
\bottomrule

\end{tabular}
% \end{small}
}
% \vspace{-0.6cm}
\end{table*}



% \begin{table*}
% \centering
% \caption{Examples of the most and least memorized training instances from SST-2 as determined by our proposed approach.
% }
% \label{table.vis.sst}
% \resizebox{\textwidth}{!}{
% % \begin{small}
% \begin{tabular}{lp{0.5cm}p{1.3cm}<{\centering}lp{0.5cm}p{1.3cm}<{\centering}}
% \toprule
% \multicolumn{3}{c}{\textbf{Negative}} & \multicolumn{3}{c}{\textbf{Positive}} \\
% \cmidrule(lr){1-3} \cmidrule(lr){4-6}
% \textbf{Content} &\textbf{Mem} & {$F(p_{k\text{NN}})$} & \textbf{Content} &\textbf{Mem} & $F(p_{k\text{NN}})$\\
% \midrule
% \begin{CJK*}{UTF8}{gbsn}
% {\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
% \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut hit} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut miss} \colorbox{red!0}{\strut affair,} \colorbox{red!0}{\strut consistently} \colorbox{red!0}{\strut amusing} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut outrageous} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut funny} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut cho} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut intended} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut imaginative} \colorbox{red!0}{\strut as} 
% \colorbox{red!0}{\strut one} 
% \colorbox{red!0}{\strut might} 
% \colorbox{red!0}{\strut have} 
% \colorbox{red!0}{\strut hoped.} 
 
% }}}
% \end{CJK*} 
% & 0.010 &  2.74 &
% \begin{CJK*}{UTF8}{gbsn}
% {\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
% \colorbox{red!0}{\strut What's} \colorbox{red!0}{\strut invigorating} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut it} 
% \colorbox{red!0}{\strut doesn't} 
% \colorbox{red!0}{\strut give} 
% \colorbox{red!0}{\strut a} 
% \colorbox{red!0}{\strut damn.} 
% }}}\end{CJK*}
% & 0.003 & 0.06 \\ 
% % \midrule
% \begin{CJK*}{UTF8}{gbsn}
% {\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
% \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut standard} \colorbox{red!0}{\strut police-oriented} \colorbox{red!0}{\strut drama} \colorbox{red!0}{\strut that,} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut deniro's} \colorbox{red!0}{\strut participation,} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut likely} \colorbox{red!0}{\strut wound} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut tnt} \colorbox{red!0}{\strut original.} 
% }}}
% \end{CJK*} 
% & 0.011 & 1.48 &
% \begin{CJK*}{UTF8}{gbsn}
% {\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
% \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut film} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut appreciated} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut those} \colorbox{red!0}{\strut willing} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut endure} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut extremely} \colorbox{red!0}{\strut languorous} 
% \colorbox{red!0}{\strut rhythms,} 
% \colorbox{red!0}{\strut waiting} 
% \colorbox{red!0}{\strut for} 
% \colorbox{red!0}{\strut happiness} 
% \colorbox{red!0}{\strut is} 
% \colorbox{red!0}{\strut ultimately} 
% \colorbox{red!0}{\strut thoughtful} 
% \colorbox{red!0}{\strut without} 
% \colorbox{red!0}{\strut having} 
% \colorbox{red!0}{\strut much} 
% \colorbox{red!0}{\strut dramatic} 
% \colorbox{red!0}{\strut impact.} 
% }}}\end{CJK*}
% & 0.010 & 0.43 \\ 
% \begin{CJK*}{UTF8}{gbsn}
% {\setlength{\fboxsep}{0pt}
% \colorbox{white!0}{\parbox{0.45\textwidth}{
% \colorbox{red!0}{\strut Although} \colorbox{red!0}{\strut god} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut great} \colorbox{red!0}{\strut addressed} \colorbox{red!0}{\strut interesting} \colorbox{red!0}{\strut matters} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut identity} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut heritage,} \colorbox{red!0}{\strut it's} \colorbox{red!0}{\strut hard} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut shake} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut feeling} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut intend} \colorbox{red!0}{\strut to} 
% \colorbox{red!0}{\strut be} 
% \colorbox{red!0}{\strut a} 
% \colorbox{red!0}{\strut different} 
% \colorbox{red!0}{\strut kind} 
% \colorbox{red!0}{\strut of} 
% \colorbox{red!0}{\strut film.} 
% }}}
% \end{CJK*} 
% & 0.066 & 1.17 
% &\begin{CJK*}{UTF8}{gbsn}
% {\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
% \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut b-movie} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut sit} \colorbox{red!0}{\strut through,} \colorbox{red!0}{\strut enjoy} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut certain} \colorbox{red!0}{\strut level} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut forget.}
% }}}\end{CJK*} 
% & 0.020 & 0.18
% \\ 
% % \midrule
% \midrule
% \begin{CJK*}{UTF8}{gbsn}
% {\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
% \colorbox{red!0}{\strut The events} \colorbox{red!0}{\strut of the film} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut just so weird} \colorbox{red!0}{\strut that}  
% \colorbox{red!0}{\strut I honestly}  
% \colorbox{red!0}{\strut never}  
% \colorbox{red!0}{\strut knew}  
% \colorbox{red!0}{\strut what}  
% \colorbox{red!0}{\strut the}  
% \colorbox{red!0}{\strut hell was}  
% \colorbox{red!0}{\strut coming}  
% \colorbox{red!0}{\strut next.}  
% }}}\end{CJK*} 
% & 0.00 & 0.00 &
% \begin{CJK*}{UTF8}{gbsn}
% {\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
% \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut colorful,} \colorbox{red!0}{\strut vibrant} \colorbox{red!0}{\strut introduction} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut universal} \colorbox{red!0}{\strut human} \colorbox{red!0}{\strut impulse,} \colorbox{red!0}{\strut lushly} \colorbox{red!0}{\strut photographed} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut beautifully} \colorbox{red!0}{\strut recorded.} 
% }}}\end{CJK*} 
% & 0.00 & 0.00 \\ 
% \begin{CJK*}{UTF8}{gbsn}
% {\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
% \colorbox{red!0}{\strut An} \colorbox{red!0}{\strut awkward} \colorbox{red!0}{\strut hybrid} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut genres} 
% \colorbox{red!0}{\strut that} 
% \colorbox{red!0}{\strut just} 
% \colorbox{red!0}{\strut doesn't} 
% \colorbox{red!0}{\strut work.} 
% }}}\end{CJK*}
% & 0.00 & 0.00 &
% \begin{CJK*}{UTF8}{gbsn}
% {\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
% \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut thought-provoking} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut often-funny} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut drama} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut isolation.} 
% }}}\end{CJK*}
% & 0.00 & 0.00
%  \\
% % \midrule
% \begin{CJK*}{UTF8}{gbsn}
% {\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
% \colorbox{red!0}{\strut Mainstream} \colorbox{red!0}{\strut audiences}
% \colorbox{red!0}{\strut will}
% \colorbox{red!0}{\strut find}
% \colorbox{red!0}{\strut little}
% \colorbox{red!0}{\strut of}
% \colorbox{red!0}{\strut interest}
% \colorbox{red!0}{\strut in}
% \colorbox{red!0}{\strut this}
% \colorbox{red!0}{\strut film,}
% \colorbox{red!0}{\strut which}
% \colorbox{red!0}{\strut is}
% \colorbox{red!0}{\strut often}
% \colorbox{red!0}{\strut preachy}
% \colorbox{red!0}{\strut and}
% \colorbox{red!0}{\strut poorly}
% \colorbox{red!0}{\strut acted.}
% }}}\end{CJK*} 
% & 0.00 & 0.00 &
% \begin{CJK*}{UTF8}{gbsn}
% {\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.45\textwidth}{
% \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut heroic} \colorbox{red!0}{\strut tale} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut persistence} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut sure} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut win} \colorbox{red!0}{\strut viewers'} \colorbox{red!0}{\strut heats.} 
% }}}\end{CJK*} 
% & 0.00 & 0.00
%  \\ 
% % \midrule
% \bottomrule

% \end{tabular}
% % \end{small}
% }
% % \vspace{-0.6cm}
% \end{table*}

